Investigating the structure and fragmentation of a highly filamentary IRDC

We present 3.7 arcsec (~0.05 pc) resolution 3.2 mm dust continuum observations from the IRAM PdBI, with the aim of studying the structure and fragmentation of the filamentary Infrared Dark Cloud G035.39-00.33. The continuum emission is segmented into a series of 13 quasi-regularly spaced (~0.18pc) cores, following the major axis of the IRDC. We compare the spatial distribution of the cores with that predicted by theoretical work describing the fragmentation of hydrodynamic fluid cylinders, finding a significant (a factor of ~8) discrepancy between the two. Our observations are consistent with the picture emerging from kinematic studies of molecular clouds suggesting that the cores are harboured within a complex network of independent sub-filaments. This result emphasizes the importance of considering the underlying physical structure, and potentially, dynamically important magnetic fields, in any fragmentation analysis. The identified cores exhibit a range in (peak) beam-averaged column density ($3.6{\rm x}10^{23}{\rm cm}^{-2}<N_{H,c}<8.0{\rm x}10^{23}{\rm cm}^{-2}$), mass ($8.1M_{\odot}<M_{c}<26.1M_{\odot}$), and number density ($6.1{\rm x}10^{5}{\rm cm}^{-3}<n_{H, c, eq}<14.7{\rm x}10^{5}{\rm cm}^{-3}$). Two of these cores, dark in the mid-infrared, centrally-concentrated, monolithic (with no traceable substructure at our PdBI resolution), and with estimated masses of the order ~20-25$M_{\odot}$, are good candidates for the progenitors of intermediate-to-high-mass stars. Virial parameters span a range $0.2<\alpha_{\rm vir}<1.3$. Without additional support, possibly from dynamically important magnetic fields with strengths of the order 230$\mu$G<B<670$\mu$G, the cores are susceptible to gravitational collapse. These results may imply a multilayered fragmentation process, which incorporates the formation of sub-filaments, embedded cores, and the possibility of further fragmentation.

==> Tex/Figures/Tex/Figure_leaf9.tex <==
\begin{figure*}
\begin{center}
\includegraphics[trim = 0mm 0mm 0mm 0mm, clip, width = 0.33\textwidth]{Tex/Figures/Figs/Figure_leaf_16_spec.png}
\includegraphics[trim = 0mm 0mm 0mm 0mm, clip, width = 0.33\textwidth]{Tex/Figures/Figs/Figure_leaf_16_mom0.png}
\end{center}
\caption{The spectral and spatial distribution of leaf~\#9. }
\label{Figure:leaf9}
\end{figure*}

==> Tex/Figures/Tex/Figure_mass_radius.tex <==
\begin{figure}
\begin{center}
\includegraphics[trim = 30mm 20mm -5mm 20mm, clip, width = 0.48\textwidth]{Tex/Figures/Figs/Figure_mass_radius16.png}
\end{center}
\caption{Cumulative enclosed mass as a function of equivalent radius (see text) for PdBI~16. The solid and dotted lines represent the flux-corrected and uncorrected masses, $M_{\rm c}$ and $M_{\rm uc}$, respectively.  The dashed line shows the predicted mass-radius relationship for a power-law density distribution with $n_{\rm c,s}~=~3.9\times10^{5}\,{\rm cm^{-2}}$ and $\kappa_{\rm \rho, c}~=~1.53\pm0.01$. The uncertainties in the radius and mass are 15 and 50 per cent, respectively. The grey shaded region signifies where the effective radius is smaller than the angular resolution of the observations. The inset image highlights the location of PdBI~16.  }
\label{Figure:mass_radius}
\end{figure}
